MV4PG: Materialized Views for Property Graphs

Graph databases are getting more and more attention in the highly interconnected data domain, and the demand for efficient querying of big data is increasing. We noticed that there are duplicate patterns in graph database queries, and the results of these patterns can be stored as materialized views first, which can speed up the query rate. So we propose materialized views on property graphs, including three parts: view creation, view maintenance, and query optimization using views, and we propose for the first time an efficient templated view maintenance method for containing variable-length edges, which can be applied to multiple graph databases. In order to verify the effect of materialized views, we prototype on TuGraph and experiment on both TuGraph and Neo4j. The experiment results show that our query optimization on read statements is much higher than the additional view maintenance cost brought by write statements. The speedup ratio of the whole workload reaches up to 28.71x, and the speedup ratio of a single query reaches up to nearly 100x.

==> sections/acknowledgment.tex <==
% \section*{Acknowledgments}
% This work was supported by Ant Group Research Fund.

==> sections/related_work.tex <==
\section{Related Work}
\label{sec:related_work}
%TODO:补充视图选择
\mysect{Materialized Views in RDBMS.} Materialized views have been studied in relational databases for several decades, and there is a great deal of work on them. ~\cite{palpanas2002incremental,himanshu2006incremental,ke2003efficient,koch2014dbtoaster,larson2006efficient} discusses the efficient maintenance of materialized views, including different kinds of views such as distributed and non-distributed aggregation functions, views containing join operators, etc.
~\cite{chaudhuri1995optimizing,halevy2000theory,flesca2001rewriting,goldstein2001optimizing} uses materialized views to reduce hits to the original database and thus optimize query efficiency, ~\cite{chaudhuri1995optimizing} discusses the timing of view optimization, suggesting that blindly using views may instead be more ineffective, ~\cite{goldstein2001optimizing} proposes a very efficient view-matching algorithm that can quickly find the right view to optimize query.
% Optimizing queries with materialized views
% 在关系型数据库中有很多物化视图相关的工作，基本的思路都是使用物化视图重写查询优化查询效率

\mysect{Materialized Views in Property Graph DBMS.} 
% 近几年也有一些图数据库物化视图的工作，~\cite{da2020kaskade}针对一个查询负载创建需要的视图，并使用视图对查询进行重写优化，重点讲述了图数据库中较为特殊的包含可变长边的查询，但是没有讨论视图维护的部分。~\cite{szarnyas2018incremental}首次提出了属性图中的增量视图维护，将图查询语句转换成关系代数的形式，使用关系型数据库中的增量维护算法，但是比较局限于理论，没有给出Evaluation的结果。
% ~\cite{han2024implementation}比较系统地讨论了属性图中的物化视图，包括增量维护和使用视图优化查询，同时也使用了一系列转换规则在关系型数据库中实现物化视图，但是并没有考虑到图数据库中比较特殊的包含可变长边的查询。
% 相比较而言，本文同时讨论了物化视图维护和使用视图优化查询两方面，并且针对于图数据库中的包含可变长边的查询给出了相应的增量维护方案，最终的实验结果也证明本文的方法起到了很大的查询速率提升。
There has also been some work on materializing views for graph databases in recent years, ~\cite{da2020kaskade} creates the required views for the workload and optimizes the query for rewriting using the views, focusing on the more specific queries in graph databases that contain variable-length edges, but not discussing the view maintenance part. ~\cite{szarnyas2018incremental} first proposed incremental view maintenance in property graphs, converting graph query statements into the form of a relational algebra, using incremental maintenance algorithms in relational databases, but is more limited to theory and does not give evaluation results.
 ~\cite{han2024implementation} discusses materialized views in property graphs more systematically, including incremental maintenance and query optimization using views, and also uses a series of transformation rules to implement materialized views in relational databases, but does not take into account the more specific queries in graph databases that contain variable-length edges.
 In contrast, this paper discusses both materialized view maintenance and query optimization using views, and gives a corresponding incremental maintenance approach for queries containing variable-length edges in graph databases, and the final experimental results also prove that this paper's method plays a great role in query rate improvement.
% Implementation Strategies for Views over Property Graphs：在图数据库上实现物化视图，查询测试不涉及可变长边

% Query rewriting for semistructured data：半结构化数据(semistructured data)的重写，给定输入为TSL(半结构化数据查询语言)和一系列视图，使用视图得到优化后的TSL查询，和我们查询重写优化的思路类似

% 关系型数据库无法迁移到图数据库的部分(Motivation?)
% 重点提图数据库查询中包含可变长的边，这是关系型数据库不具备的，并且Implementation Strategies for Views over Property Graphs文章的实验中也没有提及


